Towards Better Shale Gas Production Forecasting Using Transfer Learning

Deep neural networks can generate more accurate shale gas production forecasts in counties with a limited number of sample wells by utilizing transfer learning. This paper provides a way of transferring the knowledge gained from other deep neural network models trained on adjacent counties into the county of interest. The paper uses data from more than 6000 shale gas wells across 17 counties from Texas Barnett and Pennsylvania Marcellus shale formations to test the capabilities of transfer learning. The results reduce the forecasting error between 11% and 47% compared to the widely used Arps decline curve model.

==> backup <==


@ARTICLE{Justin,
  author  = {Montgomery, J. and Raymond, S. and O’Sullivan, F. and Williams, J},
  title   = {Shale gas production forecasting is an ill-posed inverse problem and
requires regularization},
  journal = {Upstream Oil and Gas Technology}, 
  volume  = {5},
  year    = {2020},
  doi   = {10.1016/j.upstre.2020.100022}
}




@CONFERENCE{Sun_2018,
  author  = {Sun, J. and Ma, X. and Kazi, M.},
  title   = {Comparison of Decline Curve Analysis DCA with Recursive Neural Networks RNN for Production Forecast of Multiple Wells },
  booktitle = { SPE Western Regional Meeting}, 
  year    = {2018},
  doi={https://doi.org/10.2118/190104-MS}
}


@misc{Szablowski_2020, title={What is an artificial neuron and why does it need an activation function?}, url={https://towardsdatascience.com/what-is-an-artificial-neuron-and-why-does-it-need-an-activation-function-5b4c1e971d80}, journal={Medium}, publisher={Towards Data Science}, author={Szabłowski, B.}, year={2020},
note ={Accessed: 2021-05-31}

}

@ARTICLE{Qun_2020,
  author  = {Zhao, Q. and Wang, H. and Sun, Q. and Jiang, X. and Yu, R. and Kang, L. and Wang, X.},
  title   = {A Logical Growth Model considering the influence of shale gas reservoirs
and development characteristics},
  journal = {Natural Gas Industry B}, 
  volume  = {7},
  issue = {6},
  year    = {2020},
  doi   = {https://doi.org/10.1016/j.ngib.2020.05.005}
}

@Book{ Kriesel_2007, 
       author = {Kriesel, D. }, 
       title =  { A Brief Introduction to Neural Networks },
       year =   { 2007 }, 
       url =   { available at http://www.dkriesel.com } 
     }


@ARTICLE{Justin2017,
  author  = {Montgomery, J.  and O’Sullivan, F.},
  title   = {Spatial variability of tight oil well productivity and the impact of technology},
  journal = {Applied Energy}, 
  volume  = {195},
  year    = {2017},
  doi   = {10.1016/j.apenergy.2017.03.038}
}



@ARTICLE{Lei,
  author  = {Tan, L. and Zuo, L. and Wang, B.},
  title   = {Methods of Decline Curve Analysis for Shale Gas Reservoirs},
  journal = {Energies}, 
  volume  = {11},
  year    = {2018},
  article   = {552},
  doi = {10.3390/en11030552}
}

@ARTICLE{Xia,
  author  = {Xia, Y. and Xu, T. and Yuan, Y. and Xin, X.},
  title   = {Effect of Perforation Interval Design on Gas Production from the Validated Hydrate-Bearing Deposits with Layered Heterogeneity by Depressurization},
  journal = {Geofluids, Hindawi}, 
  year    = {2020},
  doi = {10.1155/2020/8833884}
}

@ARTICLE{Manda,
  author  = {Manda, P. and Nkazi, D.},
  title   = {The Evaluation and Sensitivity of Decline Curve Modelling},
  journal = {Energies}, 
  volume  = {13},
  year    = {2020},
  article   = {552},
  pages = {2765},
  doi = {10.3390/en13112765}
}



@ARTICLE{Arps,
  author  = {Arps, J.},
  title   = {Analysis of Decline Curves},
  journal = {Transactions of the American Institute of Mining Engineers}, 
  volume  = {160},
  year    = {1945},
  doi = {10.2118/945228-G}
}


@ARTICLE{Sidel,
  author  = {Lee, W. and Sidel, R.},
  title   = {Gas reserves estimation in resource plays},
  journal = {Society of Petroleum Engineers}, 
  volume  = {2},
  doi = {10.2118/130102-PA},
  year    = {2010}
}

@ARTICLE{Leven,
  author  = {Levenberg, K.},
  title   = {A Method for the Solution of Certain Non-Linear Problems in Least Squares},
  journal = {Quarterly of Applied Mathematics}, 
  volume  = {2},
  year    = {1944},
  doi = {10.1090/qam/10666}
}

@ARTICLE{Marq,
  author  = {Marquardt, D.},
  title   = {An Algorithm for Least-Squares Estimation of Nonlinear Parameters},
  journal = {Journal of the Society for Industrial and Applied Mathematics}, 
  volume  = {11},
  year    = {1963},
  doi = {10.1137/0111030}
}

@CONFERENCE{Clark,
  author  = {Clark, A. and Lake, L. and Patzek, T.},
  title   = {Production Forecasting with Logistic Growth Models},
  booktitle = { Society of Petroleum Engineers}, 
  year    = {2011},
  doi={10.2118/144790-MS}
}


@ARTICLE{Clarkson,
  author  = {Clarkson, C. and Williams-Kovacs, J. and Qanbari, F. and Heidari Sureshjanid, M.},
  title   = {History-matching and forecasting tight/shale gas condensate wells using combined analytical, semi-analytical, and empirical methods},
  journal = {Journal of Natural Gas Science and Engineering}, 
  volume  = {26},
  year    = {2015},
  doi = {/10.1016/j.jngse.2015.03.025}
}

@ARTICLE{Lee,
  author  = {Lee, L. and Lim, J. and Yoon, D. and Jung, H.},
  title   = {Prediction of Shale-Gas Production
at Duvernay Formation Using
Deep-Learning Algorithm},
  journal = {Society of Petroleum Engineers}, 
  volume  = {24},
  year    = {2019}
}


@misc{brownlee,
  author = {Brownlee, J.},
  title  = {A Gentle Introduction to k-fold Cross-Validation},
  howpublished = "\url{https://machinelearningmastery.com/k-fold-cross-validation/}",
  year = {2020},
  note ={Accessed: 2021-05-30}
}



@ARTICLE{Han,
  author  = {Han, D. and Jung, J. and Kwon, S.},
  title   = {Comparative Study on Supervised Learning Models
for Productivity Forecasting of Shale Reservoirs
Based on a Data-Driven Approach},
  journal = {Applied Science}, 
  volume  = {10},
  year    = {2020}
}

@CONFERENCE{Li,
  author  = {Li, Y and Han, Y},
  title   = {Decline Curve Analysis for Production Forecasting Based on Machine
Learning},
  booktitle = {SPE Symposium: Production Enhancement and Cost Optimisation, Kuala Lumpur, Malaysia}, 
  year    = {2017}
}


@ARTICLE{dropout,
  author  = {Srivastava, N. and Hinton, G. and Krizhevsky, A. and Sutskever, I. and Salakhutdinov, R.},
  title   = {Dropout: A Simple Way to Prevent Neural Networks from Overfitting},
  journal = {The Journal of Machine Learning Research}, 
  volume  = {15},
  year    = {2014}
}

@ARTICLE{EIA,
  author  = {{US Energy Information Administration}},
  title   = {Oil and gas supply
module of the National Energy Modeling System 2018b},
  year    = {2018}
}


@ARTICLE{Juanes_2013,
  author  = {Cueto-Felgueroso, L. and Juanes, R.},
  title   = {Forecasting long-term gas production from shale},
  journal = {Proceedings of the National Academy of Sciences of the United States of America}, 
  year    = {2013},
  doi = {https://doi.org/10.1073/pnas.1319578110}
}

@ARTICLE{Darwesh,
  author  = {Darwesh, M.},
  title   = {The effect of perforation technology on the productivity
of hydrocarbon wells},
  journal = {Petroleum and Natural Gas Institute of
University of Miskolc}, 
  year    = {2014}
}

@misc{brownlee2,
  author = {Brownlee, J.},
  title  = {Use Early Stopping to Halt the Training of Neural Networks At the Right Time},
  howpublished = "\url{https://machinelearningmastery.com/how-to-stop-training-deep-neural-networks-at-the-right-time-using-early-stopping/}",
  year = {2019},
  note ={Accessed: 2021-05-30}
}

@misc{McKinsey_2021,
  author = {Agosta, A. and Boccara, G. and Heringa, B. and Browne, N. and Dediu, D.},
  title  = {McKinsey \& Company Global gas outlook to 2050 },
  howpublished =  "\url{https://www.mckinsey.com/industries/oil-and-gas/our-insights/global-gas-outlook-to-2050}",
  year = {2021},
  note ={Accessed: 2021-05-30}
}



@ARTICLE{Robertson,
  author  = {Robertson, S.},
  title   = {Generalized Hyperbolic Equation},
  journal = {Society of Petroleum Engineers}, 
  year    = {1988}
}



@ARTICLE{Okuszko_2008,
  author  = {Okuszko, K. and Gault, B. and Mattar, L.
},
  title   = {Production Decline Performance of CBM Wells},
  journal = {Journal of Canadian Petroleum Technology}, 
  year    = {2008},
  doi ={https://doi.org/10.2118/08-07-57}
}



@ARTICLE{Bishop,
  author  = {Bishop, C.},
  title   = {Pattern Recognition and Machine Learning},
  journal = {Springer}, 
  year    = {2006},
  ISBN    = {978-0-387-31073-2}
}

@ARTICLE{Patzek,
  author  = {Patzek, T. and Male, F. and Marder, M.},
  title   = {Gas production in the Barnett Shale obeys a simple
scaling theory},
  journal = {Proceedings of the National Academy of Sciences}, 
  year    = {2013}
}


@ARTICLE{Alfattah,
author = {Al-Fattah, S. and Startzman, R.},
year = {2001},
title = {Predicting Natural Gas Production Using Artificial Neural Network},
journal ={Society of Petroleum Engineers},
doi = {10.2118/68593-MS}
}

@ARTICLE{Duong,
author = {Duong, A.},
year = {2011},
title = {Rate-Decline Analysis for Fracture-Dominated Shale Reservoirs},
journal ={Society of Petroleum Engineers},
doi = {10.2118/137748-PA}
}

@ARTICLE{Deholanda,
author = {De Holanda, R. and Gildin, E. and Valko, P. },
year = {2018},
title = {Combining Physics, Statistics, and Heuristics in the Decline-Curve Analysis of Large Data Sets In Unconventional Reservoirs},
journal ={Society of Petroleum Engineers},
doi = {10.2118/185589-PA}
}


@CONFERENCE{Kingma,
  author  = {Kingma, D. and Ba, J.},
  title   = {Adam: A Method for Stochastic Optimization},
  booktitle = { 3rd International Conference for Learning Representations, San Diego}, 
  year    = {2017}
}

@ARTICLE{Fetkovich,
author = {Fetkovich, M.},
year = {1980},
title = {Decline Curve Analysis Using Type Curves},
journal ={Society of Petroleum Engineers},
doi = {10.2118/4629-PA}
}


@CONFERENCE{Ling2012,
  author  = {Ling, K.},
  title   = {Theoretical Bases of Arps Empirical Decline Curves},
  booktitle = {Abu Dhabi International Petroleum Conference and Exhibition, Abu Dhabi, UAE}, 
  year    = {2012}
}

@ARTICLE{Huston,
  author  = {Huston, M.},
  title   = {American Association for the Advancement of Science},
  journal = {American Association for the Advancement of Science}, 
  volume  = {359},
  year    = {2018},
  article   = {6377},
  doi = {10.1126/science.359.6377.725}
}


@misc{counties,
  author = {ERE},
  title  = {Eagle Ridge Energye},
  howpublished = "\url{http://eagleridgeenergy.com/area.php}",
  note ={Accessed: 2021-05-30}
}

@ARTICLE{YangSurvey,
  author  = {Pan, S. and Yang, Q.},
  title   = {A Survey on Transfer Learning},
  journal = {Institute of Electrical and Electronics Engineers Transactions on Knowledge and Data Engineering}, 
  volume  = {22},
  year    = {2010},
  doi ={ 10.1109/TKDE.2009.191.}
}


@book{YangBook,
place={Cambridge}, 
title={Transfer Learning},
DOI={10.1017/9781139061773},
publisher={Cambridge University Press},
author={Yang, Q. and Zhang, Y. and Dai, W. and Pan, SJ},
year={2020}
}

@book{nielsen_2020,
title={Neural Networks and Deep Learning},
author={Nielsen, M.},
year={2020},
note ={"\url{https://static.latexstudio.net/article/2018/0912/neuralnetworksanddeeplearning.pdf}" Accessed: 2021-05-30}
}

@book{Goodfellow_2016,
place={Cambridge}, 
title={Deep Learning},
ISBN={978-0262035613},
publisher={MIT Press},
author={Goodfellow, I. and Bengio, Y. and Courville, A.},
year={2016}
}



@misc{PA_website,
  author = {{Pennsylvania Department of Environmental Protection}},
  title  = {PA Oil and Gas Mapping},
  howpublished = "\url{https://www.dep.pa.gov/DataandTools/Reports/Oil\%20and\%20Gas\%20Reports/Pages/default.aspx}",
  year = 2020,
  note ={Accessed: 2021-03-30}
}

@misc{TX_website,
  author = {{Railroad Commission of Texas}},
  title  = {Online Research Queries},
  howpublished = "\url{https://www.rrc.state.tx.us/}",
  year = 2019,
  note ={Accessed: 2020-01-30}
}

@misc{EIA_website,
  author = {{US Energy Information Administration}},
  howpublished = "\url{URL: https://www.eia.gov/}",
  note ={Accessed: 2021-01-30}
}

@misc{lmfit,
  author = {Newville, M. and Stensitzki, T. and Allen, D.and Rawlik, M. and Ingargiola, A. and Nelson, A.
},
  title  = {Non-Linear Least-Squares Minimization and Curve-Fitting for Python
},
  howpublished = "\url{URL: https://lmfit.github.io/lmfit-py/}",
  year = {2020},
  note ={Accessed: 2020-01-30}
}


@ARTICLE{Hastle,
  author  = {Hastie, T. and Tibshirani, R. and Friedman, J.},
  title   = {The Elements of Statistical Learning: Data Mining, Inference, and Prediction, Second Edition},
  journal = {Springer Series in Statistics}, 
  year    = {2016},
}


@misc{Chen,
  author = {Chen, J.},
  title = {Decline Curves, investopedia},
  howpublished = "\url{https://www.investopedia.com/terms/d/decline-curve.asp}",
  year = {2018},
  note ={Accessed: 2020-07-30}
}

@misc{Bloomberg,
  author = {Merrill, D.},
  title  = {Can the U.S. Become an Energy Superpower in 2017?, Bloomberg},
  howpublished = "\url{https://www.bloomberg.com/graphics/2016-energy-pipelines/}",
  year = {2016},
  note ={Accessed: 2020-07-30}
}

@misc{brownlee3,
  author = {Brownlee, J.},
  title  = {How to Classify Photos of Dogs and Cats (with 97\% accuracy)},
  note ={"\url{https://machinelearningmastery.com/how-to-develop-a-convolutional-neural-network-to-classify-\\ photos-of-dogs-and-cats/}" Accessed: 2020-09-30},
  year = {2019}
}


@CONFERENCE{ImageNet,
  author  = {Deng, J. and Dong, W. and Socher, R. and Li, L.},
  title   = {ImageNet: a Large-Scale Hierarchical Image Database},
  booktitle = { IEEE Computer Society Conference on Computer Vision and Pattern Recognition (CVPR 2009), Miami, Florida, USA}, 
  year    = {2009}
}


@CONFERENCE{VGG,
  author  = {Zisserman, A. and Simonyan, K},
  title   = {Very Deep Convolutional Networks for Large-Scale Image Recognition},
  booktitle = {International Conference on Learning Representations , San Diego, Ca, USA}, 
  year    = {2015}
}


@ARTICLE{Mahajan,
  author  = {Mahajan, D. and Girshick, R. and Ramanathan, V. and He, K. and Paluri, M. and Li, Y. and Bharambe, A. andvan der Maaten, L},
  title   = {Exploring the Limits of Weakly Supervised Pretraining},
  journal = {CoRR}, 
  volume  = {abs/1805.00932},
  year    = {2018},
  url       = {http://arxiv.org/abs/1805.00932},
}

@misc{Zhuang,
      title={A Comprehensive Survey on Transfer Learning}, 
      author={Zhuang, F. and Qi, Z. and Duan, K. and Xi, D. and Zhu, Y. and Zhu, H. and Xiong, H. and He, Q.},
      year={2020},
      eprint={1911.02685},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}
